Toward Learning Robust and Invariant Representations with Alignment Regularization and Data Augmentation

Data augmentation has been proven to be an effective technique for developing machine learning models that are robust to known classes of distributional shifts (e.g., rotations of images), and alignment regularization is a technique often used together with data augmentation to further help the model learn representations invariant to the shifts used to augment the data. In this paper, motivated by a proliferation of options of alignment regularizations, we seek to evaluate the performances of several popular design choices along the dimensions of robustness and invariance, for which we introduce a new test procedure. Our synthetic experiment results speak to the benefits of squared l2 norm regularization. Further, we also formally analyze the behavior of alignment regularization to complement our empirical study under assumptions we consider realistic. Finally, we test this simple technique we identify (worst-case data augmentation with squared l2 norm alignment regularization) and show that the benefits of this method outrun those of the specially designed methods. We also release a software package in both TensorFlow and PyTorch for users to use the method with a couple of lines at https://github.com/jyanln/AlignReg.

==> secs/abstract.tex <==
Data augmentation has been proven to be an effective
technique for developing machine learning models 
that are 
robust to known classes of distributional shifts 
(\textit{e.g.}, rotations of images),
and this efficiency is sometimes 
interpreted as the model's learning of
representations invariant to the shifts used 
to augment the data. 
In this paper, 
motivated by an example illustrating that 
data augmentation does not necessarily lead to the learning of representations invariant to the shifts,
we first argue that the usage of alignment regularization can help achieve that goal. 
Then, with synthetic experiments and a proposed invariance test,
we evaluate the performances of several popular design options
of alignment regularizations. 
Our empirical results
speak to the benefits of 
squared $\ell_2$ norm regularization.
Further, 
we also formally analyze the behavior 
of alignment regularization
to complement our empirical study 
under assumptions we consider realistic. 
Finally, we test this simple technique over several tasks
and show that the benefits of simple data augmentation 
and alignment regularization may outrun 
those of the specially designed methods. 
% {\color{red} maybe shorten the alignment regularization to CR to save space, also check whether the term should be ``alignment regularization''}

% When facing the challenge
% of developing machine learning models 
% robust to known classes of distributional shifts
% (e.g., rotations of images), 
% data augmentation is often a handy technique. 
% While the approach has proven beneficial 
% in a variety of settings,
% the practitioner faces many 
% design choices concerning 
% how to incorporate the augmented data.
% In this paper, following the intuition 
% that training with a alignment regularization
% applied to embeddings of original data 
% and corresponding augmentations
% can help to learn robust and invariant models, 
% we study the design options
% of alignment regularizations. 
% With a proposed invariance test, 
% our experiments 
% speak to the benefits of 
% squared \ltwo{} norm alignment loss.
% Along with the empirical study, 
% we also analyze the robust error bound
% and present a complementary theoretical discussion. 
% Finally, we demonstrate 
% that across a variety of tasks,
% squared $\ell_2$ norm alignment loss
% outperforms (or is on par with) 
% several recent methods,
% each of which is specially designed for one task 
% and significantly more complicated.


==> secs/introduction.tex <==
Deep learning has achieved
remarkable empirical performance over \textit{i.i.d} test data, 
and the community continues to investigate 
more challenging scenarios 
when models are tested in robustness 
over non-\textit{i.i.d} data 
\citep[\textit{e.g.},][]{ben2010theory,szegedy2013intriguing}.  
Recent studies
suggest that one challenge of learning robust models for non-\textit{i.i.d} data 
is the model's tendency in capturing undesired features, such as the texture of the images \citep{geirhos2018imagenettrained, wang2020high, kaushik2019learning}, 
thus combating this tendency may be 
a key to learning robust models. % these arguments are probably too strong and we need fix them

To help models prevent learning these undesired features, 
data augmentation 
(\textit{i.e.}, diluting the undesired features of training samples
by applying transformations to existing examples) 
is often used \citep[\textit{e.g.},][]{Hendrycks2020augmix,goel2021model}.
It is probably one of the most common methods 
to improve model's performance.
However, 
a vanilla training with data augmentation 
may not be able to help the model to learn the desired features. 
Fortunately, a simple usage of \emph{alignment regularization} 
(AR, also known as consistency loss or consistency regularization, 
regularizing the model so that the distance between representations learned by the model 
from a pair of data will be small)
can help fix the problem 
(as illustrated in Figure~\ref{fig:intro}). 
Therefore, in this paper,
we seek to answer the question:
\emph{how should we use alignment regularization so that
the advantages of augmented data 
can be taken to the fullest extent 
to learn robust and invariant models?}

\begin{figure}
    \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/open1.png}
         \caption{vanilla training}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/open2.png}
         \caption{vanilla training with data augmentation}
     \end{subfigure}
     \begin{subfigure}[b]{0.95\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/open3.png}
         \caption{training with data augmentation and alignment regularization (AR)}
     \end{subfigure}
    \caption{A motivation of the usage of alignment regularization. Consider a typical classification problem of dog vs. cat classification where the dogs tend to be outdoor and cats tend to be indoor: (a) A vanilla training with available data may result in a model classifying the environment instead of the animals; 
    (b) A vanilla training with augmented data may result in a model that learns the classification conditioning on the environment;
    (c) If we use alignment regularization (AR) to force the model to learn same representations out of a pair of data (original sample and the augmented copy), the model is more likely to learn the classifier of the animals. 
    Given the importance of using AR, we continue to study options of the alignment regularizations in this paper.}
    \label{fig:intro}
\end{figure}

To answer this, 
we first conduct a range of experiments 
over image classification benchmarks 
to evaluate how popular variants of AR
contribute to learning robust and invariant models. 
We test for accuracy, robustness, and invariance, 
for which we propose a new test procedure.
Our empirical study favors 
squared \ltwo{} norm. 
% Further, 
% as our experiments may not be able 
% to exhaust all options, 
% we complement the empirical study
% with an analysis of 
% the generalization error bounds
% of models trained with augmented data
% and alignment regularization. 
% Our theoretical study favors $\ell_1$ norm (under assumptions introduced later). 
% With the belief that the disparity
% can be explained by the difficulties 
% in passing the gradient of $\ell_1$ norm 
% in practice, 
% we believe our formal derivations 
% can support the empirical results well. 
Further, we also complement our empirical study 
by showing that norm-based regularizations 
can lead to bounded generalization error (under assumptions introduced later). 
Our contributions of this paper are as follows: 
% Our contributions are:

\begin{itemize}
\item With a new invariance test, we show 
that while a vanilla training 
with augmented data 
can improve robustness, 
alignment regularization is important
to help the model 
learn representations 
invariant to the augmentation function, 
and squared \ltwo{} norm seems to be 
the best choice as assessed by 
a variety of empirical evaluations (\cref{sec:motivate}).  
\item On the theoretical end, 
we formalize a generalization error bound 
for models trained with AR and augmented data
% studying the worst-case expected risk over unseen data 
% when samples are allowed to be transformed 
% according to a function in a family 
(\cref{sec:method}). 
\item We test the method we identified
(squared \ltwo{} norm as AR) 
in multiple scenarios.
We believe the fact that this generic approach 
can compete with methods specially designed 
for different scenarios
can endorse its empirical strength (\cref{sec:exp}). 
\end{itemize}


% We bound the expected risk with terms 
% that can be computed during training, 
% so that our analysis can inspire 
% how to regularize the training procedure. 
% %to take full advantage of the augmentation. 
% While all the derived methods have an upper bound of the expected risk, 
% with progressively stronger assumptions, 
% we have progressively simpler regularization, 
% allowing practical choices to be made according to 
% the understanding of the application.
% %allowing us to choose the most convenient method based on the domain knowledge of the data and the augmentation in practice. 
% Our contributions of this paper are as follows: 
% \begin{itemize}
%     \item We offer analyses of the generalization behaviors of  augmented models trained with different regularizations: these regularizations require progressively stronger assumptions of the data and the augmentation functions, but progressively less computational efforts. For example, with assumptions pertaining to augmentation transformation functions, the Wasserstein distance over the original and augmented empirical distributions can be calculated through simple $\ell_1$ norm distance. 
%     \item We test and compare these methods and offer practical guidance on how to choose regularizations in practice. 
%     In short, regularizing the squared $\ell_2$ distance of logits 
%     between the augmented samples and original samples is a favorable method, 
%     suggested by both theoretical and empirical evidence. 
%     \item With an invariance test, 
%     we argue that vanilla augmentation does not 
%     utilize the augmented samples to the fullest extent, especially in learning invariant representations, 
%     thus may not be ideal unless the only goal of augmentation is 
%     to improve the accuracy over a specific setting. 
%     %of a narrow range of settings,
%     %which may not be realistic in industry. 
% \end{itemize}

% The remainder of this paper is as follows, 
% we will first briefly discussed related works about data augmentation in Section~\ref{sec:related}, 
% emphasizing training strategies instead augmenting choices.
% Then, we will present our main analysis in Section~\ref{sec:method}, 
% followed up by empirical discussion in Section~\ref{sec:exp}. 
% We will also offer some relevant discussions in Section~\ref{sec:dis}. 
% Finally, we conclude our paper in Section~\ref{sec:con} 
% by summarizing our findings in how to choose the training strategies 
% based on understandings of the data and the augmentation. 
% where we encourage the readers of empirical interest to directly go to. 
